OG-RAG: Ontology-Grounded Retrieval-Augmented Generation For Large Language Models

This paper presents OG-RAG, an Ontology-Grounded Retrieval Augmented Generation method designed to enhance LLM-generated responses by anchoring retrieval processes in domain-specific ontologies. While LLMs are widely used for tasks like question answering and search, they struggle to adapt to specialized knowledge, such as industrial workflows or knowledge work, without expensive fine-tuning or sub-optimal retrieval methods. Existing retrieval-augmented models, such as RAG, offer improvements but fail to account for structured domain knowledge, leading to suboptimal context generation. Ontologies, which conceptually organize domain knowledge by defining entities and their interrelationships, offer a structured representation to address this gap. OG-RAG constructs a hypergraph representation of domain documents, where each hyperedge encapsulates clusters of factual knowledge grounded using domain-specific ontology. An optimization algorithm then retrieves the minimal set of hyperedges that constructs a precise, conceptually grounded context for the LLM. This method enables efficient retrieval while preserving the complex relationships between entities. OG-RAG applies to domains where fact-based reasoning is essential, particularly in tasks that require workflows or decision-making steps to follow predefined rules and procedures. These include industrial workflows in healthcare, legal, and agricultural sectors, as well as knowledge-driven tasks such as news journalism, investigative research, consulting and more. Our evaluations demonstrate that OG-RAG increases the recall of accurate facts by 55% and improves response correctness by 40% across four different LLMs. Additionally, OG-RAG enables 30% faster attribution of responses to context and boosts fact-based reasoning accuracy by 27% compared to baseline methods.

==> parking.tex <==
The internet contains a vast amount of knowledge about the world across different domains such as technology~\citep{}, health~\citep{}, food~\citep{}, and news~\citep{}. Recently, large language models (LLMs) have made huge advancements in understanding human language in its raw form~\citep{}. This has led to their adoption as question-answering systems~\citep{}, search engines~\citep{}, and task-oriented chatbots~\citep{}. However, they fail to reliably generate accurate knowledge, which hinders their deployment in specific domains~\citep{}.
including healthcare~\citep{}, agriculture~\citep{}, and retail~\citep{}. 
In this work, we aim to bridge this gap by restricting the output space of the retrieved information.

While neural reasoning systems such as LLMs have been shown to be more generalizable than the earlier symbolic systems, they tend to suffer from unpredictable hallucinations~\citep{}. However, rule-based reasoning systems provide more control and interpretability to the designers, while restricting the hallucinations. Grounding the relevant facts to pre-defined keywords through an ontology would also make it easier to apply the rules that would be composed of these keywords. 

To further improve the reliability of LLMs, it is also important to find plausible sources that attributes towards a generation~\citep{}. Sources are often cited at a coarse document level, which makes it hard for users to verify the correctness~\citep{}. While more fine-grained retrieval methods have been proposed, retrieved chunks correspond to arbitrary texts in the documents which are not easy to read and verify~\citep{}. By mapping the information to certain keywords in an ontology, we can make it easier for the users to verify the correctness of the generated responses. 
Mapping this context to a common agreed-upon ontology can thus help attribute them to localized sources in a way that can be easily verified by the users.


\textbf{Parking}
To this end, we present OG-RAG, or Ontology-Grounded Retrieval Augmented Generation, that retrieves query-relevant context in the form of a pre-defined ontology of a given domain. To this end, we map/organize the domain-specific documents with respect to a given ontology and convert them into a hypergraph structure. Each node is comprised of fixed keywords and corresponding data mappings, which are filtered for a given query based on the embedding similarity with the query. Finally, the query-relevant context is formed by the minimal set of edges that cover the filtered nodes, which we add in the context of an LLM. 

However, no prior work exists that exploits this inherent domain structure for better retrieval of relevant information from domain-specific documents. \textbf{}

OG-RAG improves response accuracy, supports flexible fact-based reasoning—allowing the application of structured logic to domain and enables verifiable source attribution.


\textbf{Points to clarify}
Process based reasoning:
Process implies sequence of rules. We do not have evaluation on sequence.
While rules are very concrete, mathematical constructs and we are not quite doing that.


Large Language Models (LLMs) have demonstrated significant potential in generating human-like text across various tasks. However, a key limitation is their propensity to generate hallucinations, which are outputs that contain factually incorrect or contextually irrelevant information. Hallucinations can range from minor entity errors to entirely fabricated content, and they significantly undermine the trustworthiness of LLM outputs, especially in domains requiring high accuracy and adherence to specific processes~\citep{}. This issue is particularly important in scenarios like industrial workflows~\citep{} and knowledge work~\citep{}, where reliable adherence to defined factual rules is critical.

Efforts to mitigate hallucinations have focused on fine-grained detection and correction. Systems like \citep{} and \citep{} have been developed to identify and edit hallucinations by detecting factual errors at multiple levels, such as entity, relation, and sentence. These systems improve the factual accuracy of LLM outputs by grounding the generation process in trusted references or structured knowledge sources like ontologies. Such methods have shown promising results in reducing hallucination rates, enhancing the applicability of LLMs in domains where accuracy and factual adherence are paramount~\citep{}.

In addition to hallucination detection, improving source attribution is another critical challenge. Traditional approaches often cite sources at the document level, which can be too coarse for effective verification by users~\citep{}. More fine-grained retrieval methods, such as Retrieval-Augmented Generation (RAG), aim to address this by retrieving smaller, more relevant chunks of information~\citep{} \hlc{Maybe add about Raptor or GraphRAG here?}. However, these methods still face challenges in making the retrieved information easily interpretable and verifiable~\citep{}. By integrating ontologies, as proposed in OG-RAG, it becomes possible to precisely map domain-specific knowledge to structured entities and relationships, providing clearer attribution and making it easier for users to verify the correctness of LLM-generated responses.

Finally, rule-based reasoning systems provide greater control and interpretability compared to purely neural approaches, especially when grounded in ontologies. Rule-based systems can restrict the generation of hallucinations by ensuring that the LLM’s outputs adhere to predefined domain rules and facts~\citep{}. Combining the flexibility of LLMs with the structure of ontologies creates a hybrid approach that leverages the strengths of both systems, enabling more reliable reasoning and reducing factual errors in complex, rule-based tasks~\citep{}. 

Each domain uses certain terms that may have a different meaning outside the domain or be too niche and only used within the domain. For example, in the agriculture domain, ``Seed'' will take functional attributes such as ``grown in'', and ``requires the soil to be'', while ``Seed'' in the biological domain is likely to have attributes like ``number of leaves'' and ``get nutrients from''.

Another significant issue with LLMs is the difficulty of source attribution. Traditional retrieval models often cite sources at the document level, making it hard for users to verify the exact origin of the information~\citep{lewis2020retrieval,edge2024graphrag}. While more fine-grained attribution methods have been developed, they are restricted to finding citations and do not apply to arbitrary retrieval over documents~\citep{slobodkin2024attribute}. OG-RAG overcomes this by mapping retrieved information to structured entities within an ontology, enabling users to trace generated responses directly to specific sources and factual entities. This leads to improved transparency and trustworthiness in generated outputs.


% It would correspond to finding  particular, in the ontology, certain relationships map to $v(s, a) = \phi$ denoting that the attribute can be any sentence from the English vocabulary. We can find these va
% by setting the null value, \ie, $v(s, a) = \phi$ of each attribute $a$ of the term $s \in \CS$, such that $v(s, a) \in \CR(s, a)$ and it is equivalent to saying ``$a$ of $s$ is $v(s, a)$''. However, multiple such terms and their attributes can be set within the scope of the documents $\CD$. Thus, we can extract information $\CI:=\CD(\CO)$ as a set of self-contained \textit{info-blocks} $F \in \CD(\CO)$, where each \textit{info-block} $F$ consists of different terms having their attributes mapped to either English words or points to another object of the set $F$. More formally,
% first extract useful information from the documents  The aim is to ground the information on . use a powerful LLM to map the documents $\CD$ onto the ontology $\CO$. As mentioned in Section~\ref{sec:background}, we want to obtain a set of facts $\CD(\CO)$, where each fact represents the property named $n(a)$ of a common object $s \in \CS$ is $v_{\CD}(s, a)$. 
% We can then use the data to set the values $v(a)$ for each attribute in an ontology. This gives us

\begin{definition}[Ontology-mapped data]\label{defn:map}
    Ontology-mapped data $\CI:=\CD(\CO)$ is information derived from the documents $\CD$ using the ontology $\CO$. It is a set of info-blocks $F$, where each info-block is a set of ontology relationships such that $(s, a, v) \in F$ implies $v \in \CV$ if $v_{\CO}(s, a) = \phi$ and $v = v_{\CO}(s, a)$ otherwise. 
    % $= \{(s, a, v): \, v_{\CO}(s, a) = \phi \implies v(s, a) \in \CV\}$, where the value $v(s, a)$ either belongs to the English vocabulary $\CV$ or is recursively defined using other elements of the same info-block, \ie, $(a(s), a', v') \in F$ for some $a', v'$.
\end{definition}
    % $= \{(s, a, v): \, v_{\CO}(s, a) = \phi \implies v(s, a) \in \CV\}$, where the value $v(s, a)$ either belongs to the English vocabulary $\CV$ or is recursively defined using other elements of the same info-block, \ie, $(a(s), a', v') \in F$ for some $a', v'$.



\begin{algorithm}[t]
    \caption{Flattening a factual block}
    \label{alg:flatten}
    \begin{algorithmic}[1]
        \Require{Factual block $F$, Concatenation operator $\oplus$.
        % Ontology-mapped data $\CI$,
        }
        \Ensure{A set of flattened factual-blocks $\overline{F} \gets \, $\Call{Flatten}{$F$} flattens any nested information present in $F$.}
        \Procedure{Flatten}{$F$}
            \State $\overline{F} \gets \{\}$
            % \For{$F \in X$}
            \State $\overline{F}_0 
            \gets \{(s, a, v) \in F: v \in \CV, (s', a', s) \notin F\}$. \Comment{top-level}
            \State $\overline{F} \gets \overline{F} \cup \{\overline{F}_0\}$.
            \For{$(s, a, v) \in F \backslash \overline{F}_0$}.
                \If{$v \in \CS$} % \notin \CV$}
                    \State $F_v \gets \overline{F}_0 \cup \{(s \oplus a \oplus v, a', v'): (v, a', v') \in F\}$.
                    % , v' \in \CV\}$
                    % \State $\overline{\CX} \gets \overline{\CX} \cup \{F'\}$
                    \State $\overline{F} \gets \overline{F} \;  \cup \, $ \Call{Flatten}{$F_v$}. \Comment{flatten nesting of $v$}
                    % \ElsIf{$v \subset \CS$}
                    %     \For{$v_i \in v$}
                    %         \State $F' \gets \overline{F} \cup \{(s \oplus a \oplus v_i, a', v'): (v_i, a', v') \in F\}$.
                    %         \State $\overline{X} \gets \overline{X} \;  \cup \, $ \Call{Flatten}{$\{F'\}$}.
                    %     \EndFor
                    \EndIf
                \EndFor 
            % \EndFor
            \State \Return{$\overline{F}$}
        \EndProcedure
        % \State Flattened factual-blocks 
        % \For{$F \in \CI$}
        %     \State $\overline{\CI} \gets$ \{\Call{Flatten}{F, \{\}}\}
        % \EndFor
            % \State $\overline{F} 
            % \gets \{(s, a, a(s)) \in F: a(s) \in \CV, (s', a', s) \notin F\}$.
    \end{algorithmic}
\end{algorithm}


% in which case, step 4, we would call \textsc{Flatten} at most $d_{\CO}$ times and each call would take at most 

% Note that each factual-block is . Let us denote the time taken by \textsc{Flatten} as $T(\CI)$, then we have $T(\CI) = |\CI|(|F|_{max} T)$ for 

% These rules are curated since they represent knowledge that is not explicitly mentioned in the documents and thus, needs to be deduced by applying these rules in the appropriate context. 

% These prompts are made as long as we generate the desired number of questions that are above a threshold rating. Furthermore, we pick $5$ randomly sampled chunks from the domain-specific data in each iteration. We thus generate $10$ such questions with at least $7$ rating.

% the generated question is sent to another LLM call to generate the correct answer and then, finally, to another LLM to give the question a rating using the prompt
% \begin{center}
%     {\small\texttt{
%         Given the following data and a set of deductive rules, check if the given question requires the application of the rules on the data to generate the given answer. Rate the question from 1-10, where 10 denotes a very good application of the rules and 1 denotes a bad application of the rules. 
%         Print the reasoning as "Reasoning: <>" followed by the rating as "Rating: <rating>", where <rating> is an integer from 1-10. \\
%         Data: \textcolor{gray}{< Domain-specific data >} \\
%         Rules: \textcolor{gray}{< Fixed set of rules >} \\
%         Question: \textcolor{gray}{< Generated question >} \\
%         Answer: \textcolor{gray}{< Generated answer >} \\
%         Reasoning: \\
%         Rating:
%     }}
% \end{center}
% 


% To address these gaps, we present OG-RAG, which introduces fact-based context retrieval to dynamically adapt LLM responses to specific domain requirements, improving response accuracy. OG-RAG further enables factual deduction, enhancing reasoning by allowing the system to infer conclusions based on established domain knowledge. Additionally, OG-RAG provides improved context attribution, ensuring transparent and reliable verification by tracing responses back to their underlying facts. These contributions collectively enable OG-RAG to adapt to domain-specific needs, improving accuracy and transparency in LLM responses.
% \hlc{Edit this by adding results. Our evaluations in the agriculture and news domains demonstrate that OG-RAG improves context recall by 20\% and response accuracy by 15\%. Our user study shows that attributing LLM responses to the context retrieved by OG-RAG is faster and easier. Finally, in a fact-based reasoning task, we find that LLMs are better able to apply pre-defined facts or rules when reasoning over OG-RAG's context compared to other methods.}
